UniAP: Unifying Inter- and Intra-Layer Automatic Parallelism by Mixed Integer Quadratic Programming

Distributed learning is commonly used for training deep learning models, especially large models. In distributed learning, manual parallelism (MP) methods demand considerable human effort and have limited flexibility. Hence, automatic parallelism (AP) methods have recently been proposed for automating the parallel strategy optimization process. Existing AP methods suffer from sub-optimal solutions because they do not jointly optimize the two categories of parallel strategies (i.e., inter-layer parallelism and intra-layer parallelism). In this paper, we propose a novel AP method called UniAP, which unifies inter- and intra-layer automatic parallelism by mixed integer quadratic programming. To the best of our knowledge, UniAP is the first parallel method that can jointly optimize the two categories of parallel strategies to find an optimal solution. Experimental results show that UniAP outperforms state-of-the-art methods by up to 3.80$\times$ in throughput and reduces strategy optimization time by up to 107$\times$ across five Transformer-based models.

==> sec/6_impact_statement.tex <==

%\section*{Impact Statement}\label{sec:impact-statement}
%This paper proposes UniAP to advance the field of deep learning infrastructure.
%We have not found immediate ethical concerns or negative societal consequences of our work.
%Therefore, none of the negative consequences must be specifically highlighted.

%However, training a Transformer-based model often requires a significant amount of energy.
%UniAP depicts the opportunity to greatly accelerate the training process, thereby minimizing energy consumption as much as possible.
%Hence, we feel the necessity to highlight its positive environmental impact here.
% Therefore, we do not feel the necessity to highlight them here.

